Topic Ontologies for Arguments

Many computational argumentation tasks, like stance classification, are topic-dependent: the effectiveness of approaches to these tasks significantly depends on whether the approaches were trained on arguments from the same topics as those they are tested on. So, which are these topics that researchers train approaches on? This paper contributes the first comprehensive survey of topic coverage, assessing 45 argument corpora. For the assessment, we take the first step towards building an argument topic ontology, consulting three diverse authoritative sources: the World Economic Forum, the Wikipedia list of controversial topics, and Debatepedia. Comparing the topic sets between the authoritative sources and corpora, our analysis shows that the corpora topics-which are mostly those frequently discussed in public online fora - are covered well by the sources. However, other topics from the sources are less extensively covered by the corpora of today, revealing interesting future directions for corpus construction.

==> table-classification.tex <==
\begin{table*}
\centering
\scriptsize
\setlength{\tabcolsep}{2pt}
\begin{tabular}{@{}l@{\hspace{10\tabcolsep}}cccc@{\hspace{4\tabcolsep}}cccc@{\hspace{4\tabcolsep}}cccc@{\hspace{4\tabcolsep}}cccc@{\hspace{4\tabcolsep}}cccc@{}}
\toprule
\bf Approach & \multicolumn{8}{@{}c@{\hspace{4\tabcolsep}}}{\bf World Economic Forum} & \multicolumn{8}{@{}c@{\hspace{4\tabcolsep}}}{\bf Wikipedia} & \multicolumn{4}{@{}c@{}}{\bf \kern-2pt Debatepedia\kern-2pt} \\
\cmidrule(r{4\tabcolsep}){2-9}\cmidrule(r{4\tabcolsep}){10-17}\cmidrule{18-21}
& \multicolumn{4}{@{}c@{\hspace{4\tabcolsep}}}{Level 1} & \multicolumn{4}{@{}c@{\hspace{4\tabcolsep}}}{Level 2} & \multicolumn{4}{@{}c@{\hspace{4\tabcolsep}}}{Level 1} & \multicolumn{4}{@{}c@{\hspace{4\tabcolsep}}}{Level 2} \\
\cmidrule(r{4\tabcolsep}){2-5}\cmidrule(r{4\tabcolsep}){6-9}\cmidrule(r{4\tabcolsep}){10-13}\cmidrule(r{4\tabcolsep}){14-17}
Baselines & & P & R & F & & P & R & F & & P & R & F & & P & R & F & & P & R & F \\
\midrule
Random & & 0.02 & 0.02 & 0.02 & & 0.01 & 0.01 & 0.01 & & 0.11 & 0.11 & 0.11 & & 0.01 & 0.01 & 0.01 & & 0.07 & 0.07 & 0.07 \\
Direct match & & 0.38 & 0.23 & 0.29 & & 0.59 & 0.11 & 0.19 & & 0.12 & 0.04 & 0.06 & & 0.47 & 0.34 & 0.40 & & 0.49 & 0.37 & 0.42 \\
\addlinespace
By threshold & $\mathbf{\theta}$ & P & R & F & $\mathbf{\theta}$ & P & R & F & $\mathbf{\theta}$ & P & R & F & $\mathbf{\theta}$ & P & R & F & $\mathbf{\theta}$ & P & R & F \\
\midrule
SI & 0.02 & 0.18 & 0.63 & 0.28 & 0.02 & 0.20 & 0.58 & 0.29 & 0.01 & 0.29 & 0.51 & 0.37 & 0.05 & 0.54 & 0.64 & \bf 0.59 & 0.02 & 0.52 & 0.61 & \bf 0.56 \\
SI-lemma & 0.03 & 0.20 & 0.47 & 0.28 & 0.02 & 0.19 & 0.59 & 0.29 & 0.01 & 0.29 & 0.48 & 0.36 & 0.05 & 0.51 & 0.67 & 0.58 & 0.02 & 0.51 & 0.59 & 0.55 \\
W2V-SI & 0.20 & 0.14 & 0.63 & 0.23 & 0.16 & 0.13 & 0.63 & 0.21 & 0.10 & 0.12 & 0.55 & 0.20 & 0.11 & 0.18 & 0.69 & 0.29 & 0.07 & 0.29 & 0.81 & 0.43 \\
SI$_{\mathrm{GloVe}}$ & 0.98 & 0.14 & 0.61 & 0.22 & 0.98 & 0.12 & 0.66 & 0.21 & 0.97 & 0.14 & 0.59 & 0.23 & 0.96 & 0.15 & 0.83 & 0.25 & 0.98 & 0.32 & 0.71 & 0.44 \\
T2V-SI$_{\mathrm{ELMo}}$ & 0.87 & 0.18 & 0.32 & 0.23 & 0.80 & 0.13 & 0.65 & 0.22 & 0.74 & 0.23 & 0.45 & 0.31 & 0.76 & 0.25 & 0.45 & 0.32 & 0.87 & 0.47 & 0.46 & 0.47 \\
T2V-SI$_{\mathrm{BERT}}$ & 0.94 & 0.19 & 0.39 & 0.25 & 0.93 & 0.15 & 0.49 & 0.23 & 0.92 & 0.36 & 0.22 & 0.27 & 0.89 & 0.22 & 0.52 & 0.31 & 0.92 & 0.36 & 0.64 & 0.46 \\
SI$_{\mathrm{flair}}$ & 0.96 & 0.15 & 0.38 & 0.22 & 0.98 & 0.24 & 0.18 & 0.21 & 0.89 & 0.14 & 0.45 & 0.22 & 0.86 & 0.15 & 0.82 & 0.25 & 0.93 & 0.30 & 0.71 & 0.42 \\
SI$_{\mathrm{WGloVe}}$ & 0.99 & 0.14 & 0.37 & 0.21 & 0.99 & 0.12 & 0.39 & 0.19 & 0.92 & 0.11 & 0.86 & 0.20 & 0.93 & 0.14 & 0.88 & 0.25 & 0.57 & 0.26 & 0.98 & 0.41 \\
SI$_{\mathrm{WELMo}}$ & 0.83 & 0.16 & 0.39 & 0.23 & 0.78 & 0.13 & 0.57 & 0.22 & 0.73 & 0.24 & 0.32 & 0.27 & 0.71 & 0.22 & 0.54 & 0.31 & 0.83 & 0.40 & 0.51 & 0.45 \\
SI$_{\mathrm{WBERT}}$ & 0.91 & 0.15 & 0.50 & 0.24 & 0.93 & 0.15 & 0.43 & 0.22 & 0.89 & 0.18 & 0.35 & 0.24 & 0.87 & 0.20 & 0.55 & 0.30 & 0.92 & 0.37 & 0.54 & 0.44 \\
SI$_{\mathrm{Wflair}}$ & 0.90 & 0.13 & 0.66 & 0.21 & 0.97 & 0.17 & 0.23 & 0.20 & 0.82 & 0.12 & 0.74 & 0.20 & 0.78 & 0.14 & 0.96 & 0.25 & 0.91 & 0.30 & 0.69 & 0.42 \\
\addlinespace
By rank & k & P & R & F & k & P & R & F & k & P & R & F & k & P & R & F & k & P & R & F \\
\midrule
SI & \phantom{0}12 & 0.22 & 0.75 & 0.34 & \phantom{0}30 & 0.21 & 0.68 & 0.32 & \phantom{00}3 & 0.32 & 0.65 & 0.43 & \phantom{0}12 & 0.39 & 0.70 & 0.50 & \phantom{0}19 & 0.43 & 0.78 & \bf 0.56 \\
SI-lemma & \phantom{0}11 & 0.23 & 0.74 & \bf 0.35 & \phantom{0}33 & 0.21 & 0.70 & \bf 0.33 & \phantom{00}3 & 0.30 & 0.60 & 0.40 & \phantom{0}19 & 0.36 & 0.76 & 0.49 & \phantom{0}21 & 0.42 & 0.77 & 0.55 \\
W2V-SI & \phantom{0}83 & 0.13 & 0.94 & 0.24 & 439 & 0.12 & 0.77 & 0.21 & \phantom{0}14 & 0.11 & 1.00 & 0.20 & 290 & 0.16 & 0.77 & 0.27 & \phantom{0}61 & 0.27 & 0.86 & 0.42 \\
SI$_{\mathrm{GloVe}}$ & 119 & 0.11 & 1.00 & 0.21 & 822 & 0.10 & 1.00 & 0.18 & \phantom{00}5 & 0.19 & 0.66 & 0.30 & 705 & 0.14 & 1.00 & 0.25 & \phantom{0}18 & 0.33 & 0.66 & 0.44 \\
T2V-SI$_{\mathrm{ELMo}}$ & \phantom{00}4 & 0.25 & 0.44 & 0.32 & \phantom{0}42 & 0.13 & 0.68 & 0.23 & \phantom{00}2 & 0.39 & 0.53 & 0.45 & \phantom{0}46 & 0.18 & 0.64 & 0.28 & \phantom{0}13 & 0.43 & 0.71 & 0.54 \\
T2V-SI$_{\mathrm{BERT}}$ & \phantom{00}7 & 0.19 & 0.53 & 0.28 & \phantom{0}80 & 0.11 & 0.66 & 0.20 & \phantom{00}2 & 0.41 & 0.55 & \bf 0.47 & \phantom{0}80 & 0.17 & 0.70 & 0.28 & \phantom{0}23 & 0.36 & 0.80 & 0.50 \\
SI$_{\mathrm{flair}}$ & 109 & 0.11 & 0.99 & 0.21 & 820 & 0.10 & 1.00 & 0.18 & \phantom{00}6 & 0.17 & 0.68 & 0.27 & 692 & 0.14 & 0.99 & 0.25 & \phantom{0}77 & 0.26 & 0.97 & 0.41 \\
SI$_{\mathrm{WGloVe}}$ & 137 & 0.11 & 1.00 & 0.20 & 822 & 0.10 & 1.00 & 0.18 & \phantom{0}11 & 0.13 & 0.93 & 0.23 & 748 & 0.14 & 1.00 & 0.24 & \phantom{0}83 & 0.26 & 0.98 & 0.41 \\
SI$_{\mathrm{WELMo}}$ & \phantom{00}7 & 0.18 & 0.53 & 0.27 & \phantom{0}63 & 0.13 & 0.73 & 0.22 & \phantom{00}3 & 0.30 & 0.62 & 0.41 & \phantom{0}28 & 0.18 & 0.55 & 0.27 & \phantom{0}16 & 0.40 & 0.76 & 0.53 \\
SI$_{\mathrm{WBERT}}$ & \phantom{0}12 & 0.15 & 0.56 & 0.24 & 822 & 0.10 & 1.00 & 0.18 & \phantom{00}2 & 0.38 & 0.51 & 0.44 & \phantom{0}83 & 0.16 & 0.69 & 0.27 & \phantom{0}22 & 0.36 & 0.77 & 0.49 \\
SI$_{\mathrm{Wflair}}$ & 137 & 0.11 & 1.00 & 0.20 & 820 & 0.10 & 1.00 & 0.18 & \phantom{00}9 & 0.14 & 0.82 & 0.24 & 748 & 0.14 & 1.00 & 0.24 & \phantom{0}84 & 0.25 & 1.00 & 0.41 \\
\bottomrule
\end{tabular}
\caption{Performance of explicit topic modeling approaches in human evaluation for each topic ontology level in terms of precision (P), recall (R), and F$_1$-score (F) for the ``relevant'' label. For methods other than the baselines the table shows the values for both the similarity threshold~$\theta$ and rank~$k$ that lead to the highest F$_1$-score respectively. The best F$_1$-scores for each ontology are marked in bold. The T2V methods that employ GloVe, flair, and/or weighting consistently performed worse than the others and are omitted from the table for clarity.}
\label{table-classification}
\end{table*}


==> table-top-topics.tex <==
\begin{table}[t]
\centering
\scriptsize
\setlength{\tabcolsep}{1pt}
\begin{tabular}{@{}lc@{}}
\multicolumn{2}{@{}l@{}}{(a) World Economic Forum}\\
\toprule
{\bfseries Topic} (Level~1) & \bfseries Units\\
\midrule
1 4th Industrial Rev. & 695,473 (1.19\%) \\
2 Fut. Econ. Progr.   & 693,350 (1.19\%) \\
3 Future of Mobility  & 691,202 (1.19\%) \\
4 AI and Robotics     & 687,033 (1.16\%) \\
5 Values              & 684,393 (1.16\%) \\
\bottomrule
\end{tabular}%
\hfill%
\begin{tabular}{@{}lc@{}}
\multicolumn{2}{@{}l@{}}{(b) Wikipedia}\\
\toprule
{\bfseries Topic} (Level~2) & \bfseries Units\\
\midrule
1 Church-state-sep. & 227,377 (1.73\%)  \\
2 Meaning of life   & 186,486 (1.42\%) \\
3 Creation science  & 161,624 (1.23\%) \\
4 Women's right     & 152,284 (1.16\%) \\
5 Christian right   & 141,246 (1.08\%)\\
\bottomrule
\end{tabular}%
\hfill%
\begin{tabular}{@{}lc@{}}
\multicolumn{2}{@{}l@{}}{(c) Debatepedia} \\
\toprule
{\bfseries Topic} (Level~1) & \bfseries Units\\
\midrule
1 Politics           & 636,841 (5.31\%)  \\
2 United States          & 584,899 (4.88\%) \\
3 Law           & 417,620 (3.48\%) \\
4 Society         & 357,368 (2.98\%) \\
5 Morality       & 307,462 (2.56\%)\\
\bottomrule
\end{tabular}%
\hfill%
\raisebox{-10ex}[0em][0em]{\raisebox{20ex}[0em][0em]{(d) Wikipedia}\kern-6em\includegraphics{histogram-arguments-per-topic-wikipedia}}
\caption{The distribution of the documents in all argument corpora in Table \ref{table-argument-corpora} on the identified topics in Wikipedia, World Economic Forum, and Debatepedia using SI and the best corresponding threshold.}
\label{table-top-topics}
\end{table}


==> table-topic-matching-analysis.tex <==
\begin{table}[t]
\centering
\scriptsize
\setlength{\tabcolsep}{1pt}
\begin{tabular}{@{}lccccc@{}}
\toprule
\multicolumn{1}{l}{\bf Topic Ontology} & \multicolumn{1}{l}{ \bf Corpora Topics} & \multicolumn{4}{c}{ \bf Ontology Topics}\\
\cmidrule{3-6}
                  &     & All & Min & Mean & Max\\
\midrule
WEF Level 1       & 461 &  75 & 1 & 1.42 &  5 \\
WEF Level 2       & 131 &  52 & 1 & 1.36 &  4 \\
Wikipedia Level 1 & 561 & 185 & 1 & 1.68 &  6 \\
Wikipedia Level 2 & 516 &  13 & 1 & 1.20 &  3 \\
Debatepedia       & 761 &  82 & 1 & 2.98 & 10 \\
\bottomrule
\end{tabular}%
\caption{The count of matched corpora topics, ontology topics, and the (minimum, mean, and maximum) count of matched ontology topics per corpus topic.}
\label{table-topic-matching-anlaysis}
\end{table}


==> table-topic-ontologies.tex <==
\begin{table}
\centering
\scriptsize
\setlength{\tabcolsep}{3pt}
\begin{tabular}{@{}l@{\hspace{3\tabcolsep}}cccc@{}}
\toprule
\bf Ontology & \bf Curators & \bf Scope & \multicolumn{2}{c}{\bf Topics} \\
\cmidrule(l{\tabcolsep}){4-5}
             &                &                           &       Level 1 & Level 2 \\
\midrule
WEF          & Domain experts & Domestic \& global topics &           137 &     822 \\
Wikipedia    & Wiki editors   & Controversial articles    & \phantom{0}14 &     748 \\
Debatepedia  & Wiki editors   & Public discourse          & \phantom{0}89 &      -- \\
\bottomrule
\end{tabular}
\caption{Comparison of the employed topic ontologies.}
\label{table-topic-ontologies}
\end{table}

%\begin{table*}
%\centering
%\scriptsize
%\setlength{\tabcolsep}{2pt}
%\begin{tabular}{@{}l@{\hspace{4\tabcolsep}}ccc@{\hspace{2\tabcolsep}}cc@{\hspace{6\tabcolsep}}ccc@{\hspace{2\tabcolsep}}ccc@{\hspace{2\tabcolsep}}ccc@{\hspace{2\tabcolsep}}cc@{}}
%\toprule
%\bf Ontology & \bf Curators & \bf Scope & \multicolumn{3}{@{}c@{\hspace{6\tabcolsep}}}{\bf Documents} & \bf Lvl. & \multicolumn{10}{@{}c}{\bf Topics} \\
%\cmidrule(r{6\tabcolsep}l{\tabcolsep}){4-6}\cmidrule(l{\tabcolsep}){8-17}
% & & & Genre & \# & Authors & & \# & \multicolumn{3}{@{}c@{\hspace{2\tabcolsep}}}{Authors} & \multicolumn{3}{@{}c@{\hspace{2\tabcolsep}}}{Documents} & \multicolumn{3}{@{}c@{\hspace{2\tabcolsep}}}{Tokens} \\
%\cmidrule(r{2\tabcolsep}l{2\tabcolsep}){9-11}\cmidrule(r{2\tabcolsep}l{2\tabcolsep}){12-14}\cmidrule(l{2\tabcolsep}){15-17}
% & & & & & & & & Min & Mean & Max & Min & Mean & Max & Min & Mean & Max \\
%\midrule
%\multirow{2}{*}{WEF} & \multirow{2}{*}{\shortstack{Domain\\experts}} & \multirow{2}{*}{\shortstack{Domestic \&\\global topics}} & \multirow{2}{*}{\shortstack{News\\articles}} & \multirow{2}{*}{9,600} & \multirow{2}{*}{\phantom{00}6,270} & 1 & 137 & \phantom{0,00}1 & \phantom{0,0}334.1 & \phantom{00}1,787 & \phantom{00}3 & 940.7 & 4,080 & \phantom{00,}945 & 490,576.6 & 2,950,615 \\
% & & & & & & 2 & 822 & \phantom{0,00}1 & \phantom{0,0}216.8 & \phantom{00}1,300 & \phantom{00}1 & 550.3 & 3,337 & \phantom{00,}251 & 310,229.7 & 2,292,371 \\
%\addlinespace[3pt]
%\multirow{2}{*}{Wikipedia} & \multirow{2}{*}{Editors} & \multirow{2}{*}{\shortstack{Controversial\\articles}} & \multirow{2}{*}{\shortstack{Encyclop.\\articles}} & \multirow{2}{*}{\phantom{0,}748} & \multirow{2}{*}{823,682} & 1 & \phantom{0}14 & 9,124 & 78,013.7 & 225,623 & \phantom{0}11 & \phantom{0}68.0 & \phantom{0,}172 & 26,977 & 339,088.0 & 1,198,813 \\
% & & & & & & 2 & 748 & \phantom{0,00}9 & \phantom{0}1,929.5 & \phantom{0}13,810 & \phantom{00}1 & \phantom{00}1.0 & \phantom{0,00}1 & \phantom{00,00}6 & \phantom{00}6,149.1 & \phantom{0,0}22,116 \\
%\addlinespace[3pt]
%Debatepedia & Editors & Pub.\ discourse & Discussions & 5,489 & \phantom{00}1,815 & - & \phantom{0}89 & \phantom{0,0}12 & \phantom{0,0}145.0 & \phantom{000,}682 & \phantom{00}7 & \phantom{0}61.7 & \phantom{0,}306 & \phantom{0}2,987 & \phantom{0}84,787.6 & \phantom{0,}475,033 \\
%\bottomrule
%\end{tabular}
%\caption{Comparison of the employed topic ontologies by curators, scope, and associated documents, and of their levels by their topic statistics. Documents with unknown author are ignored for the author statistics.}
%\label{table-topics-ontologies}
%\end{table*}

%\begin{table*}[t]
%\centering
%\scriptsize
%\setlength{\tabcolsep}{4.3pt}
%\caption{The number of topics and topic statistics for each level of the three ontologies discussed in this paper. Documents with unknown author are ignored for the author statistics.}
%\label{table-topics-ontologies}
%\vspace{1ex}
%\begin{tabular}{@{}l@{\hspace{4\tabcolsep}}c@{\hspace{3\tabcolsep}}ccc@{\hspace{3\tabcolsep}}ccc@{\hspace{3\tabcolsep}}ccc@{}}
%\toprule
%\bf Topic Ontology & \bf Topics & \multicolumn{9}{@{}c}{\bf Topic Statistics} \\
%\cmidrule{3-11}
% & & \multicolumn{3}{@{}c@{\hspace{3\tabcolsep}}}{Authors} & \multicolumn{3}{@{}c@{\hspace{3\tabcolsep}}}{Documents} & \multicolumn{3}{@{}c@{\hspace{3\tabcolsep}}}{Tokens} \\
%\cmidrule(r{3\tabcolsep}){3-5}\cmidrule(r{3\tabcolsep}){6-8}\cmidrule{9-11}
%      &     & Min         & Mean           & Max           & Min       & Mean        & Max         & Min          & Mean            & Max             \\
%\midrule
%World Economic Forum Level 1 &           137 & \phantom{0,00}1 & \phantom{0,0}334.1 & \phantom{00}1,787 & \phantom{00}3 &           940.7 &           4,080 & \phantom{00,}945 &           490,576.6 &           2,950,615 \\
%World Economic Forum Level 2 &           822 & \phantom{0,00}1 & \phantom{0,0}216.8 & \phantom{00}1,300 & \phantom{00}1 &           550.3 &           3,337 & \phantom{00,}251 &           310,229.7 &           2,292,371 \\
%Wikipedia Level 1            & \phantom{0}14 &           9,124 &           78,013.7 &           225,623 & \phantom{0}11 & \phantom{0}68.0 & \phantom{0,}172 &           26,977 &           339,088.0 &           1,198,813 \\
%Wikipedia Level 2            &           748 & \phantom{0,00}9 & \phantom{0}1,929.5 & \phantom{0}13,810 & \phantom{00}1 & \phantom{00}1.0 & \phantom{0,00}1 & \phantom{00,00}6 & \phantom{00}6,149.1 & \phantom{0,0}22,116 \\
%Debatepedia             & \phantom{0}89 & \phantom{0,0}12 & \phantom{0,0}145.0 & \phantom{000,}682 & \phantom{00}7 & \phantom{0}61.7 & \phantom{0,}306 & \phantom{0}2,987 & \phantom{0}84,787.6 & \phantom{0,}475,033 \\
%\bottomrule
%\end{tabular}
%\vspace{-4ex}
%\end{table*}

